Quantitative study of the AMS-02 electron/positron spectra: implications for the pulsar and dark matter properties

The AMS-02 has just published the unprecedentedly precise measurement of the cosmic electron and positron spectra. In this paper we try to give a quantitative study on the AMS-02 results by a global fitting to the electron and positron spectra, together with the updated positron fraction data. The Markov Chain Monte Carlo algorithm is adopted to do the fitting. The primary electron spectrum and the parameters for pulsars or dark matter which contribute extra positrons are determined simultaneously. We find that there is a hardening of the primary electron spectrum at $\sim 60$ GeV. With such a new feature at the background spectrum both the pulsars and dark matter can explain the AMS-02 results very well. The dark matter scenario shows a drop at positron fraction at $\sim 300$ GeV, however, suffers very strong constraints from Fermi $\gamma$-ray observations. The fitting results also suggest that the propagation model with convection may be more favored by the lepton data than the reacceleration model.

==> tab/limit.tex <==
\begin{tabular}{*{10}{c}}
\hline
\rule[-5.25pt]{0pt}{15pt} &  & \multirow{2}{*}{$\dfrac{\chi^2}{\mathrm{d.o.f.}}$} & \multirow{2}{*}{$\chi^2$} & \multirow{2}{*}{$\dfrac{e^+}{e^++e^-}$} & \multirow{2}{*}{$e^-$} & \multirow{2}{*}{$e^+$} &$\log(A_\mathrm{psr}\footnote{Pre-propagated normalization of pulsar injection at $1\MeV$ in unit $\cm^{-3}\s^{-1}\MeV^{-1}$.})$ & $\alpha$ & $\log(R_\mathrm{c}/\MeV)$ \\
\cline{8-10}
\rule[-5.25pt]{0pt}{15pt}& & & && & & $\log(\langle \sigma v\rangle\footnote{In unit $\cm^3\s^{-1}$})$ & $\log(m_\chi/\GeV)$ & ---\\
\hline
\multirow{3}{*}{DR} & PSR & 2.45 & 475.1 & 235.0 & 63.21 & 176.9 & -23.04 & 2.289 & 8.496\\
 & $\mu$ & 27.7 & 5402.0 & 2050.0 & 1049.0 & 2303.0 & -24.13 & 2.083 & --\\
 & $\tau$ & 13.5 & 2625.0 & 1071.0 & 433.1 & 1121.0 & -23.43 & 2.32 & --\\
\hline
\multirow{3}{*}{DC} & PSR & 0.863 & 167.4 & 70.53 & 30.73 & 66.16 & -24.78 & 1.964 & 9.579\\
 & $\mu$ & 12.2 & 2370.0 & 852.1 & 402.4 & 1116.0 & -23.89 & 2.241 & --\\
 & $\tau$ & 5.54 & 1080.0 & 367.5 & 208.6 & 503.7 & -23.13 & 2.558 & --\\
\hline
\end{tabular}


==> tab/prior.tex <==
\begin{tabular}{*{9}{c}}
\hline
\rule[-8.399999999999999pt]{0pt}{24.0pt} &  & $\dfrac{\chi^2}{\mathrm{d.o.f.}}$ & $\dfrac{\chi^2_\mathrm{data}}{\mathrm{d.o.f.}}$ & $\chi^2_\mathrm{data}$ & $\chi^2_\varphi$ & $c_{e^+}$ & $\varphi$ \\[1ex]
\hline
\multirow{3}{*}{DR} & psr & 1.57 & 0.72 & 191.5 & 226.1 & 2.957 & 1.131\\
 & $\mu$ & 1.66 & 0.719 & 191.9 & 252.1 & 3.145 & 1.169\\
 & $\tau$ & 1.56 & 0.661 & 176.5 & 241.0 & 3.08 & 1.153\\
\hline
\multirow{3}{*}{DC} & psr & 0.859 & 0.673 & 179.1 & 49.44 & 1.344 & 0.606\\
 & $\mu$ & 2.39 & 1.36 & 363.8 & 273.7 & 1.929 & 0.7414\\
 & $\tau$ & 1.48 & 0.808 & 215.7 & 178.5 & 1.789 & 0.6961\\
\hline
\end{tabular}

